A high-contrast coronagraph for earth-like exoplanet direct imaging: design and test

The high-contrast coronagraph for direct imaging earth-like exoplanet at the visible needs a contrast of 10^(-10) at a small angular separation of 4 lambda/D or less. Here we report our recent laboratory experiment that is close to the limits. The test of the high-contrast imaging coronagraph is based on our step-transmission apodized filter. To achieve the goal, we use a liquid crystal array (LCA) as a phase corrector to create a dark hole based on our dedicated focal dark algorithm. We have suppressed the diffracted and speckle noise near the star point image to a level of 1.68 x 10^(-9) at 4 lambda/D, which can be immediately used for the direct imaging of Jupiter like exoplanets. This demonstrates that high-contrast coronagraph telescope in space has the potentiality to detect and characterize earth-like planets.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

